LangNav: Language as a Perceptual Representation for Navigation

We explore the use of language as a perceptual representation for vision-and-language navigation (VLN), with a focus on low-data settings. Our approach uses off-the-shelf vision systems for image captioning and object detection to convert an agent's egocentric panoramic view at each time step into natural language descriptions. We then finetune a pretrained language model to select an action, based on the current view and the trajectory history, that would best fulfill the navigation instructions. In contrast to the standard setup which adapts a pretrained language model to work directly with continuous visual features from pretrained vision models, our approach instead uses (discrete) language as the perceptual representation. We explore several use cases of our language-based navigation (LangNav) approach on the R2R VLN benchmark: generating synthetic trajectories from a prompted language model (GPT-4) with which to finetune a smaller language model; domain transfer where we transfer a policy learned on one simulated environment (ALFRED) to another (more realistic) environment (R2R); and combining both vision- and language-based representations for VLN. Our approach is found to improve upon baselines that rely on visual features in settings where only a few expert trajectories (10-100) are available, demonstrating the potential of language as a perceptual representation for navigation.

==> prompts/few_shot.tex <==
\begin{quote}
    \texttt{You are a navigation agent who must navigate according to instructions given only descriptions of your current position via natural language. The natural language description is sometimes incorrect.\\
\\
At each step, you will be given several directions and captions for each direction. You must choose one direction by printing only the [caption\_of\_the\_direction] or choose "Stop" if you think the goal is reached.\\
\\
For example:\\
\\
Input:\\
\\
To your [direction\_1] is, [caption of the direction\_1].\\
......\\
To your [direction\_N] is, [caption of the direction\_N].\\
\\
You choose:\\
\\
Output: [caption of the direction\_3]\\
\\
And here is an example trajectory:\\
\\
\#\#\# Instruction:\\
Go down the stairs. Turn right and go down the hallway. Turn right and stand near the fireplace.\\
\\
\#\#\# Trajectory:\\
Step 1:\\
\\
To your straight ahead is,\\
an ornate doorway leading to another room\\
\\
To your 60 degree right is,\\
a red carpeted staircase leading to a chandelier\\
\\
To your 120 degree right is,\\
a room with a red carpet and a large mirror\\
\\
To your back and 30 degree down is,\\
a room with a red carpet and two windows\\
\\
To your 120 degree left is,\\
a room with a red carpet and gold trim\\
\\
You chose:\\
a room with a red carpet and gold trim\\
\\
Step 2:\\
\\
To your 150 degree right is,\\
a very ornate staircase in a house with red and white striped chairs\\
\\
To your back is,\\
a red carpeted hallway leading to a staircase\\
\\
To your 150 degree left is,\\
a hallway with a red carpet and a chandelier\\
\\
To your 120 degree left is,\\
a room with a red carpet and a chandelier\\
\\
To your 90 degree left is,\\
a room with a chandelier and two windows\\
\\
To your 60 degree left is,\\
a room with a red carpet and a large mirror\\
\\
To your 30 degree right is,\\
a hallway with a red carpet and wooden doors\\
\\
You chose:\\
a hallway with a red carpet and wooden doors\\
\\
Step 3:\\
\\
To your back is,\\
a hallway with a red carpet and a chandelier\\
\\
To your straight ahead is,\\
a hallway with a red carpet and a gold ceiling\\
a hallway with a red carpet and a gold ceiling\\
\\
You chose:\\
a hallway with a red carpet and a gold ceiling\\
\\
Step 4:\\
\\
To your 90 degree right is,\\
a living room with a chandelier and a fireplace\\
\\
To your 120 degree right is,\\
a room with a fireplace and a chandelier in it\\
\\
To your back is,\\
a hallway with a red carpet and gold trim\\
\\
To your 90 degree left is,\\
a room with a chandelier and a table in it\\
\\
To your 30 degree right is,\\
a living room with a chandelier and a couch\\
\\
You chose:\\
a living room with a chandelier and a fireplace\\
\\
Step 5:\\
\\
To your straight ahead is,\\
a living room filled with furniture and a fire place\\
\\
To your 30 degree left is,\\
a living room filled with furniture and a chandelier\\
\\
To your 150 degree right is,\\
a room with a chandelier and a table in it\\
\\
To your back is,\\
a hallway with a chandelier and a mirror on the wall\\
\\
To your 90 degree left is,\\
a living room filled with furniture and a chandelier\\
\\
You chose:\\
\\
Stop\\
\\
Hint: You should use the information inside the instructions, history steps, and current observations to make the decision.\\
\\
Now let's start!}
\end{quote}


==> prompts/full_r2r_examples.tex <==
\begin{quote}
\texttt{You are a navigation agent who must navigate according to instructions given only descriptions of your current position via natural language. The natural language description is sometimes incorrect. \\  \\ \#\#\# Instruction: \\ Go across the kitchen passed the pizza oven into the next room. Stop just inside the bedroom.  \\  \\ \#\#\# Trajectory: \\ Step 1: \\  \\ To your 60 degree left is,  \\ a kitchen with a stove, sink, and refrigerator \\ Details:  oven, bowl, dining table, microwave, refrigerator \\  \\ To your 30 degree left is,  \\ a kitchen with white cabinets and a white stove top oven \\ Details:  oven, bowl, microwave, potted plant, chair \\  \\ To your 60 degree right is,  \\ a living room filled with furniture and a fire place \\ Details:  couch, chair \\  \\ To your back is,  \\ a room with a bed and a painting on the wall \\  \\ You chose: \\ a living room filled with furniture and a fire place \\  \\ Step 2: \\  \\ To your 150 degree left is,  \\ a kitchen with a stove top oven sitting next to a counter \\ Details:  oven, dining table, microwave, refrigerator, chair \\  \\ To your back is,  \\ a kitchen with a wooden table and white appliances \\ Details:  oven, bowl, dining table, microwave, refrigerator, apple, couch, chair \\  \\ To your 30 degree right is,  \\ a living room with a couch a chair and a window \\ Details:  couch \\  \\ To your 120 degree right is,  \\ a dining room table with a bowl of fruit on it \\ Details:  chair, bowl, dining table \\  \\ To your 150 degree right is,  \\ a bowl of fruit sits on a wooden table \\ Details:  couch, chair, bowl, dining table \\  \\ You chose: \\ a living room with a couch a chair and a window \\  \\ Step 3: \\  \\ To your back is,  \\ a kitchen with a table, chairs, and stairs \\ Details:  oven, dining table, refrigerator, potted plant, chair \\  \\ To your 150 degree right is,  \\ a room with a table, chairs, and stairs \\ Details:  oven, chair, refrigerator, dining table \\  \\ To your straight ahead and 30 degree down is,  \\ a view of a hallway from the top of stairs \\ Details:  refrigerator \\  \\ To your 90 degree right and 30 degree up is,  \\ a room with a staircase and a mirror on the wall \\ Details:  toilet \\ \\ You chose: \\ a view of a hallway from the top of stairs \\  \\ Step 4: \\  \\ To your back and 60 degree up is,  \\ a living room filled with furniture and a ceiling fan \\ Details:  oven, potted plant, refrigerator \\  \\ To your 90 degree left and 30 degree up is,  \\ a living room with a couch and a table \\  \\ To your straight ahead and 30 degree up is,  \\ a bedroom with a bed and a mirror on the wall \\ Details:  bed \\  \\ You chose: \\ a bedroom with a bed and a mirror on the wall \\  \\ Step 5: \\  \\ To your back is,  \\ a hallway leading to a kitchen and living room \\ Details:  refrigerator, potted plant \\  \\ To your 30 degree left is,  \\ a room with a wooden door and a mirror \\  \\ To your straight ahead is,  \\ a bedroom with a bed, dresser, mirror and a ceiling fan \\ Details:  potted plant, bed \\  \\ To your 30 degree right is,  \\ a bedroom with a bed and a ceiling fan \\ Details:  potted plant, bed \\  \\ To your 60 degree right is,  \\ a bedroom with a bed, dresser and mirror \\ Details:  potted plant, bed \\  \\ You chose: \\ stop}
\end{quote}


==> prompts/phase_1.tex <==
\begin{quote}
    \texttt{I am going to give you example instructions written by humans to train a deep learning-based navigation agent acting inside a home. These example instructions are intended to be completed by the navigation agent in 5-7 steps. \\
    - \{real\_instruction\_1\} \\
    - \{real\_instruction\_2\} \\
    - \{real\_instruction\_3\} \\
    Your goal is to write 10 more instructions like the above that can be used to train a navigation agent. Since the navigation agent will be navigating in different home environments, your instructions should also be diverse and cover a wide range of home environments and rooms. You should make sure that the instruction can be completed by an agent in 5 to 7 steps.}
\end{quote}

% \begin{prompt}[Prompt for generating synthetic instructions (Phase I)]
% \begin{systemmessage}
% I am going to give you example instructions written by humans to train a deep learning-based navigation agent acting inside a home. These example instructions are intended to be completed by the navigation agent in 5-7 steps.
% \end{systemmessage}

% \begin{fewshotexamples}
% \begin{usermessage}
% JSON:

% \begin{jsonblock}
% ```json
% {
%     "data": {
%         "home_line": {
%             "name": "Magic",
%             "city": "Orlando",
%             "wins": 6,
%             "losses": 9,
%             "pts": 92,
%             "pts_qtr1": 18,
%             "pts_qtr2": 28,
%             "pts_qtr3": 21,
%             "pts_qtr4": 25,
%             "fg_pct": 45,
%             "fg3_pct": 19,
%             "ft_pct": 70,
%             "ast": 18,
%             "reb": 44,
%             "tov": 14
%         },
%         "visitor_line": {
%             "name": "Heat",
%             "city": "Miami",
%             "wins": 7,
%             "losses": 6,
%             "pts": 99,
%             "pts_qtr1": 22,
%             "pts_qtr2": 27,
%             "pts_qtr3": 19,
%             "pts_qtr4": 31,
%             "fg_pct": 52,
%             "fg3_pct": 46,
%             "ft_pct": 72,
%             "ast": 17,
%             "reb": 33,
%             "tov": 16
%         },
%         "box_score": {
%             "luol_deng": {
%                 "player_name": "Luol Deng",
%                 "first_name": "Luol",
%                 "second_name": "Deng",
%                 "city": "Miami",
%                 "start_position": "F",
%                 "min": 33,
%                 "pts": 9,
%                 "fgm": 4,
%                 "fga": 9,
%                 "fg_pct": 44,
%                 "fg3m": 1,
%                 "fg3a": 2,
%                 "fg3_pct": 50,
%                 "ftm": 0,
%                 "fta": 0,
%                 "ft_pct": 0,
%                 "reb": 7,
%                 "oreb": 1,
%                 "dreb": 6,
%                 "ast": 0,
%                 "stl": 1,
%                 "blk": 0,
%                 "to": 2,
%                 "pf": 3
%             },
%             ...
%         } 
%     }
% }
% ```
% \end{jsonblock}

% Write a summary of the game described above.
% \end{usermessage}

==> prompts/phase_2.tex <==
\begin{quote}
    \texttt{Here is an example of a large language model acting as a blind navigation agent in an indoor environment through text descriptions. The agent is given an instruction at the start and must follow the instruction. At each time step, the agent is given descriptions of its field of view via the following template:\\
\\
To your [VIEW] is [CAPTION]\\
-  [VIEW] consists of the agent's visible field of view (e.g., 30 degrees right, 120 degrees left, etc.)\\
- [CAPTION] is the text description of that view obtained from an image captioning model \\
\\
\#Example 1 \\
\#\#\# Instruction: \{real\_instruction\_example\} \\
\#\#\# Trajectory: \{real\_trajectory\_example\} \\
\\
Now I will give you another instruction. Please generate a trajectory of 5-7 steps that would complete the instruction. \\
\#Example 2\\
\#\#\# Instruction: \{synthetic\_instruction\}
}
\end{quote}

==> prompts/zero_shot.tex <==
\begin{quote}
    \texttt{You are a navigation agent who must navigate according to instructions given only descriptions of your current position via natural language. The natural language description is sometimes incorrect.\\
\\
At each step, you will be given several directions and captions for each direction. You must choose one direction by printing only the [caption\_of\_the\_direction] or choose "Stop" if you think the goal is reached.\\
\\
For example:\\
\\
Input:\\
\\
To your [direction\_1] is, [caption of the direction\_1].\\
......\\
To your [direction\_N] is, [caption of the direction\_N].\\
\\
You choose:\\
\\
Output: [caption of the direction\_3]\\
\\
Hint: You should use the information inside the instructions, history steps, and current observations to make the decision.}
\end{quote}

==> sections/4_experiment.tex <==
\begin{figure*}
\centering
\vspace{-6mm}
\includegraphics[width=0.8\linewidth]{figures/task_gaps.pdf}
\vspace{-2mm}
\caption{Task gap between ALFRED and R2R. We highlight notable distinctions between the navigation tasks in ALFRED and R2R, encompassing variations in appearance, step size, and instruction complexity. See \cref{sec:sim} for more details.}
\vspace{-4mm}
\label{fig:gap}
\end{figure*}


\vspace{-1mm}
\section{Empirical Study with LangNav} \label{sec:exp}
\vspace{-1mm}

Our empirical experiments are not intended to improve the state-of-the-art on VLN but are more intended to assess whether  performing  vision-language navigation with text-only language models is at all feasible, and  whether language can serve as a more {transferable} and domain-invariant perceptual representation for VLN. We first introduce the main VLN task and evaluation metrics used in our experiments (\cref{sec:task}). We then discuss the two  experiments on transferring navigation knowledge via language from synthetic trajectories obtained from the ALFRED simulated environment (\cref{sec:sim}) and GPT-4 (\cref{sec:gpt4}). We also compare our method with  previous vision-feature-based methods to show that our method generalizes better to new, unseen environments in R2R (\cref{sec:vis}).

\vspace{-1mm}
\subsection{Datasets and Metrics}\label{sec:task}
\vspace{-1mm}
\paragraph{R2R dataset.} Our core experiments are on the Room-to-Room (R2R) dataset~\cite{anderson2018vision}, a realistic vision-and-language navigation dataset consisting of 21,567 navigation instructions in the Matterport3D~\cite{anderson2018vision} environment. The R2R task requires an agent to use instructions and observations to make decisions during navigation. The dataset includes 90 scenes, with 61 scenes in the train and validation ``seen'' sets, and 11 scenes in the validation ``unseen'' set. The validation seen set shares the same set of scenes with the train set but with different instructions and trajectories. The performance on the validation seen set reflects how well the agent can navigate in a scene that has observed before, whereas the performance on the unseen set tests for generalization to completely new environments.

\vspace{-2mm}
\paragraph{Metrics.} We use the standard R2R task performance metrics.
\textit{Trajectory Length} (\texttt{TL}): the average path length in meters. \textit{Navigation Error} (\texttt{NE}): the average distance between the agent's final position and the goal in meters. \textit{Success Rate} (\texttt{SR}): the ratio of trajectories in which the agent stopped within 3 meters of the goal. \textit{Oracle Success Rate} (\texttt{OSR}): the ratio of trajectories in which the agent stopped within 3 meters to the goal with a view of the goal, \textit{Success} weighted by the normalized inverse of the \textit{Path Length} (\texttt{SPL})~\cite{anderson2018evaluation}.


\begin{table*}[t]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular*}{1.017\textwidth}{|c|c|c|c|c|c|c|c|c|c|c|c|c}
\cline{1-12}
\multirow{2}{*}{\textsc{\# Train}} & \multirow{2}{*}{\textsc{Approach}}  & \multicolumn{5}{c|}{\textit{R2R Seen}} & \multicolumn{5}{c|}{\textit{R2R Unseen}} \\ 
\cline{3-12}
 &  & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{OSR$\uparrow$} & \texttt{SPL$\uparrow$} & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{OSR$\uparrow$} & \texttt{SPL$\uparrow$}  \\ 
\hline
\hline
0 & \textsc{Rand. walk} & 7.9 & 10.2 & 2.5 & 5.1 & 1.4 & 7.6 & 9.5 & 2.9 & 5.7 & 1.9 \\
\hline
\hline
4.7K & \textsc{VL Seq2seq} & 11.0 & 8.0 &  27.1 & 36.7 & - &  10.7 & 8.6 & 19.6 & 29.1 & -  \\
\hline
\hline
\multirow{2}{*}{\textit{0 (0\%)}} & \textsc{VLN Bert} &  20.7 & 9.5 & 8.4 & 11.8 & 3.5 & 22.0 & \textbf{9.0} & 6.9 & 12.1 & 2.7 \\
\cline{2-12}
  & \textsc{Blind Agent} &  9.0 & \textbf{9.2} & \textbf{16.9} & \textbf{20.3} & \textbf{15.3} & 8.9 & 9.1 & \textbf{18.1} & \textbf{24.2}  & \textbf{16.0} \\
\hline
\hline
\multirow{2}{*}{\textit{10 (0.2\%)}} & \textsc{VLN Bert} & 10.6 & 11.3 & 8.4 & 19.4 & 7.4 &  11.6 & 11.0 & 10.2 & \textbf{23.1} & 8.7 \\
\cline{2-12}
  & \textsc{Blind Agent} &  8.1 & \textbf{8.7} & \textbf{18.5} & \textbf{20.1} & \textbf{17.7} &  8.1 & \textbf{8.3} & \textbf{18.4} & 21.4 & \textbf{17.2} \\
\hline
\hline
 \multirow{2}{*}{\textit{100 (2\%)}} & \textsc{VLN Bert} &  9.5 & 9.3 & 19.6 & 25.6 & 17.6 &  9.9 & 9.2 &  17.5 & 26.4 & 15.6 \\
\cline{2-12}
  & \textsc{Blind Agent} &  8.5 & \textbf{8.1} & \textbf{25.4} & \textbf{29.4} & \textbf{23.8} & 8.5 & \textbf{8.0} & \textbf{24.3} & \textbf{28.9} & \textbf{22.4} \\
\cline{1-12}
\end{tabular*}
}
\vspace{-2mm}
\caption{
Sim2real transfer, where we pretrain on the synthetic ALFRED environment and transfer to the real R2R environment. In this table, {\textsc{\# Train}} is the number of training examples used in the R2R environment. We present the results of our  \textbf{zero-shot sim2real} experiments (0\%) and our \textbf{few-shot learning} experiments conducted at various training sizes (0.2\% and 2\%).}
\vspace{-3mm}
\label{tab:sim}
\end{table*}

\subsection{Language-based Sim2Real Transfer}\label{sec:sim}

Our first experiment is on using language to transfer embodied knowledge from a simulated synthetic environment (ALFRED) to the realistic R2R dataset. We first begin by discussing the significant difference between the ALFRED task trajectories and the R2R task trajectories. Then we conduct the sim2real experiments where we transfer the navigation knowledge from ALFRED to R2R. 

\paragraph{ALFRED dataset.} The ALFRED dataset, based on the AI2THOR environment~\cite{ai2thor}, provides language instructions for household tasks. These instructions include a high-level goal instruction and step-by-step instructions written by humans, as show in \cref{fig:gap}. The benchmark consists of 120 scenes, with 108 scenes allocated to the train, validation seen, and test seen sets, 4 scenes for the validation unseen set, and 8 scenes for the test unseen set. 


\paragraph{Difference between ALFRED and R2R.} 
% After filtering interaction trajectories, significant task gaps remain between ALFRED's synthetic navigation trajectories and the realistic trajectories from R2R. 
There are significant differences between ALFRED and R2R which makes straightforward sim2real transfer challenging. These differences include:
\begin{itemize}
    \vspace{-2mm}
    \item \textsc{Visual appearance:} ALFRED uses images rendered from the synthetic AI2THOR environment, while R2R, based on the Matterport3D, incorporates images captured from real indoor environments. These image sources differ in texture, occlusion, illumination, and other visual aspects.
    \vspace{-2mm}
    \item \textsc{Step size:} There is a  difference in step sizes between the two tasks (see the right part of \cref{fig:gap}). ALFRED uses a step size of $0.25$ meters, while R2R has larger and more variable step sizes. To bridge this gap, we consolidate four consecutive \texttt{MoveAhead} steps into a single step along the ALFRED trajectory.
    \vspace{-2mm}
    \item \textsc{Action type:} A complete ALFRED trajectory includes not only navigation actions but also interaction actions, where the interaction actions are combined with a target object to change the state of the surrounding environment. In order to filter the interaction actions in ALFRED, we divide each ALFRED trajectory into multiple sub-trajectories and keep the sub-trajectories that are labeled with the \texttt{GotoLocation} tag.
    \vspace{-2mm}
    \item \textsc{Instruction complexity:} Due to trajectory splitting, ALFRED's navigation trajectories and instructions appear simpler and shorter compared to R2R's instructions. R2R instructions involve guiding the agent between rooms, whereas ALFRED trajectories mainly keep the agent within a single room.
    \vspace{-2mm}
    \item \textsc{Action space:} In ALFRED, the agent is limited to rotating left/right by $90\degree$ and moving forward, while in R2R, the agent can move in any combination of 12 candidate heading directions and 3 elevation directions. The number of available movement directions is irregular. This difference in action space makes R2R trajectories more human-like. To address this, we introduce randomness by adding or reducing a heading offset of $\pm 30\degree$ to the agent's direction at each step in ALFRED, allowing rotations of $30\degree$ or $60\degree$ in addition to $90\degree$.
\end{itemize}

\begin{figure*}
\centering
\vspace{-5mm}
\includegraphics[width=0.95\linewidth]{figures/pipeline_of_generating.pdf}
% \vspace{-4mm}
\caption{Pipeline for generating trajectories from a prompted GPT-4. In Phase I, we prompt GPT-4 with 3 randomly sampled navigation instructions $U$ to generate 10 more synthetic navigation instructions. Then in Phase II, for each generated navigation instruction, we prompt GPT-4 to generate the trajectory that fulfills the generated instruction. See \cref{appx:temp} for details.}
\vspace{-6mm}
\label{fig:pipeline}
\end{figure*}



\vspace{-1mm}
\subsubsection{Experimental Setup} 
% \vspace{-1mm}

To investigate the ability to learn from simulated data, we conduct the sim2real experiments where we use trajectories from the synthetic ALFRED environment as pretraining data and either use it in R2R directly (zero-shot) or finetune on a small number of R2R trajectories (few-shot). We pretrain on 128K ALFRED instruction-following pairs whose format is given in \cref{sec:prompt}. We augment the observations in ALFRED to 12 views and randomly mask a variable number of views to mimic the irregular number of candidates in R2R. See \cref{sec:imp} for the full experimental setup.
\paragraph{Baselines.} We compare our \textsc{Blind Agent} against the following baselines:
\begin{itemize}
    \vspace{-2mm}
    \item \textsc{Random Walk:} The random-walk agent randomly selects an action from the action space $\mathcal{A}_t$ at each time step, where $a_t \sim \pi^r = \frac{1}{|\mathcal{A}_t|}$. The agent can choose one of the navigable directions to move or choose to stop.
    \vspace{-2mm}
    \item \textsc{VLN Bert:} This baseline uses traditional vision-based features to parameterize a VLN agent. We similarly pretrain on simulated data and then finetune on R2R. To align with the action space in R2R, we augment the visual observations in ALFRED by expanding from one view to twelve views, covering a panoramic view. We incorporate trajectory history by concatenating the sequence of selected view features from previous steps into the input sequence of the model. The imitation learning algorithm described before is utilized to optimize the model.
    \vspace{-2mm}
    \item \textsc{VL Seq2seq (Teacher-Force):} Additionally  we include the full seq2seq model presented in \cite{anderson2018vision}, which is pretrained on the R2R train dataset, for comparison with our method. This model, which also uses vision-based features,  learns via  behavior cloning on teacher demonstrations. This approach is not directly comparable to the above transfer learning methods since it uses a far larger R2R dataset. However, with the performance results on the validation unseen set, we provide insight into the sim2real performance vs. a fully-supervised method.
\end{itemize}
\vspace{-2mm}
\paragraph{Results.}
 The  results are shown in \cref{tab:sim}. We find that our language-based transfer with the blind language model agent (\textsc{Blind Agent})  demonstrates a significant improvement over the vision-feature-based method in the sim2real scenario, in both the zero-shot and the few-shot settings. When considering the success rate, our approach performs comparably to the model that is fully pre-trained with the R2R training set on the R2R validation unseen benchmark.  This outcome suggests that language can act as an invariant perceptual representation for embodied navigation tasks. 
\begin{figure*}
\centering
% \vspace{-5mm}
\includegraphics[width=0.95\linewidth]{figures/spot_check.pdf}
% \vspace{-5mm}
\caption{An example of a generated trajectory from GPT-4. The example demonstrates a generated trajectory by following the pipeline in \cref{fig:pipeline}, where an embodied agent follows the instruction and locates the bookshelf. See more examples in \cref{appx-gen}.}
% \vspace{-4mm}
\label{fig:spot}
\end{figure*}

% \vspace{-1mm}
\subsection{Learning from GPT-4-Generated Trajectories}\label{sec:gpt4}
% \vspace{-1mm}
Experiments in \cref{sec:sim} indicate that our approach can effectively learn from the simulated environment through language-based transfer learning. However, while transfer learning from simulated environments can reduce the cost of collecting realistic data, they still require extensive human annotations for demonstration trajectories and manual designs of the indoor layout. 

We next explore a more extreme setting where we do not even assume access to a simulated environment and purely rely on GPT-4~\cite{openai2023gpt4} to generate entire  trajectories, including instructions, observations, and actions. We posit that large language models like GPT-4 have been exposed to enough text that describes taking actions within an embodied environment such that it can generate trajectories that  do not violate physics (most of the time).  Here we are in the few-shot setting where we assume access to a few R2R trajectories with which to prompt GPT-4.


\begin{table*}[t]
\centering

\resizebox{\textwidth}{!}{
\begin{tabular*}{1.03\textwidth}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \toprule
\cline{1-13}
\multirow{2}{*}{\textsc{\# real}} & \multirow{2}{*}{\textsc{\# syn.}} & \multirow{2}{*}{\textsc{src}}  & \multicolumn{5}{c|}{\textit{R2R Seen}} & \multicolumn{5}{c|}{\textit{R2R Unseen}} \\ 
% \cmidrule(lr){3-7} \cmidrule(lr){8-12}  
\cline{4-13}
 &  & & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{OSR$\uparrow$} & \texttt{SPL$\uparrow$} & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{OSR$\uparrow$} & \texttt{SPL$\uparrow$}  \\ 
% \midrule
\hline
\hline
10 & \multirow{2}{*}{0} & \multirow{2}{*}{N/A} &   11.4 & 10.3 & 9.5 & 16.9 & 7.6 & 11.4 & 9.8 & 10.7 & 20.2 & 8.4\\
\cline{1-1} \cline{4-13}
100 & & &  9.4 & 9.0 & 19.7 & 25.0 & 18.0 & 9.9 & 9.2 &  16.8 & 24.5 & 15.1 \\
% \cline{1-13}
\hline
\hline
10 & \multirow{2}{*}{21K} & \multirow{2}{*}{ALFRED} &  8.1 & 8.7 & 18.5 & 20.1 & 17.7 &  8.1 & 8.3 & 18.4 & 21.4 & 17.2\\
\cline{1-1} \cline{4-13}
100 & & & 8.5 & \textcolor{brown}{\textbf{8.1}} & \textcolor{brown}{\textbf{25.4}} & \textcolor{brown}{\textbf{29.4}} & \textcolor{brown}{\textbf{23.8}} & 8.5 & \textcolor{brown}{\textbf{8.0}} & 24.3 & 28.9 & 22.4 \\
% \cline{1-13}
\hline
\hline
% 10 & 50 & 9.6 & 9.6 & 11.4 & 19.7 & 9.7 & 9.5 & 9.4 & 13.3 & 20.6 & 11.3 \\
% 10 & 100 &  10.5 & 9.6 & 13.2 & 23.1 & 10.8 & 10.4 & 9.0 & 17.0 & 28.6 & 14.4\\
10 & \multirow{2}{*}{0.5K} & \multirow{2}{*}{GPT-4} & 9.1 & \textcolor{blue}{\textbf{8.2}} & \textcolor{blue}{\textbf{21.3}} & \textcolor{blue}{\textbf{26.8}} & \textcolor{blue}{\textbf{18.9}} & 9.0 & \textcolor{blue}{\textbf{7.9}} & \textcolor{blue}{\textbf{22.6}} & \textcolor{blue}{\textbf{29.9}} & \textcolor{blue}{\textbf{20.7}} \\
\cline{1-1} \cline{4-13}
100 & & &  9.2 & 8.2 & 25.0 & \textcolor{brown}{\textbf{29.4}} & 23.3 & 9.5 & 8.1 & \textcolor{brown}{\textbf{25.7}} & \textcolor{brown}{\textbf{33.6}} & \textcolor{brown}{\textbf{23.3}} \\
\cline{1-13}
\end{tabular*}
}

\caption{
Results from learning from GPT-4 generated trajectories. The column headers provide the following information: \textsc{\# real} represents the number of real R2R trajectories for finetuning the agent, \textsc{\# syn.} indicates the number of synthetic trajectories, and \textsc{src} denotes the source of the synthetic trajectories (ALFRED vs. GPT-4). The best results of 10-shot and 100-shot are marked in \textcolor{blue}{\textbf{blue}} and \textcolor{brown}{\textbf{brown}} respectively.}
\label{tab:gpt4}
\end{table*}

\paragraph{Generating trajectories.}
We generate all of the synthetic trajectories by using only 10 real trajectories from the R2R train set. Each real trajectory has 3 navigation instructions which are narrated by 3 different annotators. Thus we have 30 navigation instructions $\{U^{(i)}\}_{i=1}^{30}$ in total. The entire pipeline can be divided into two phases. In phase I, for each prompt, we randomly choose 3 real instructions as prompt examples and ask GPT-4 to write 10 more instructions like the examples, as is shown in \cref{fig:pipeline}.\footnote{It is possible that GPT-4 training set included the instructions seen in R2R. However, out of the 500 generated instructions, we find 0 of them were seen in the R2R dataset. Note that while instructions may have been encountered, the trajectories were unlikely to have been encountered during pretraining since we used vision systems to obtain the captions/objects.} We collect 500 generated navigation instructions in this phase. Then in phase II, for each generated instruction, we prompt GPT-4 to generate a trajectory to fulfill the instruction, conditioned on a real demonstration instruction and trajectory. The real trajectory is obtained by obtaining the trajectory whose instruciton is closest to the synthetic instruction based on the CLIP~\cite{radford2021learning} text features. We instruct GPT-4 to  complete the trajectory in 5-7 steps.  

We present an illustrative example in \cref{fig:spot} to demonstrate the benefits of the generated trajectory. Following the pipeline depicted in \cref{fig:pipeline}, we first generate an instruction, such as \texttt{``Enter the hallway [...]"} and then prompt GPT-4 to generate a trajectory that fulfills the given instruction. Upon analyzing the examples, we have identified three key aspects that indicate the high quality of the generated trajectories:
\begin{itemize}
    \item \textsc{Strong Prior:} The generated scenarios exhibit a strong adherence to real-world room-object and object-object correlations, as evident from descriptions like ``\texttt{a bathroom with a sink, mirror, [...]}'' and ``\texttt{a kitchen with modern appliances and a countertop.}'' 
    % \vspace{-2mm}
    \item \textsc{Spatial Consistency:} The example reveals spatial consistency within the generated trajectories. For instance, in \texttt{Step 4}, the agent correctly identifies the door with a potted plant, consistent with its position in \texttt{Step 3}. Such instances emphasize the preservation of spatial relationships across the generated trajectories.
    % \vspace{-2mm}
    \item \textsc{Descriptive:} The generated trajectories incorporate a significant amount of  captions and objects that do not directly relate to the given instruction, which plays a crucial role in preparing the agent to navigate successfully in real-world scenarios.
\end{itemize}

\paragraph{Results.}
We adopt a similar approach as before and use the generated trajectories as pretraining data. The results of this approach are shown in \cref{tab:gpt4}. By incorporating these trajectories, our method successfully enhances the navigation performance on R2R. We conduct a comparative analysis with the outcomes obtained from learning with simulated trajectories in ALFRED, where we find that 500 synthetic trajectories from GPT-4 can almost match the performance of transferring from 21K trajectories from ALFRED. The comparison demonstrates that learning from GPT-4-generated trajectories not only delivers superior navigation performance but also exhibits a significantly higher level of data efficiency.

\subsection{Generalization to Unseen Rooms} \label{sec:vis}
Finally, \cref{tab:comp_vis} presents a comparison between our method and state-of-the-art vision-feature-based methods where we use the full R2R training set to train our blind naviation agent. While our approach does not surpass the best systems, it exhibits a significant reduction in the discrepancy between the validation seen set and the validation unseen set, indicating that using language as the perceptual representation enhances the ability to generalize navigation across unfamiliar scenes. See the \cref{appx:r2r} for full results.


\begin{table}[t]
\centering

\begin{tabular}{|c|c|c|c|}%{lllllll}
\cline{1-4}
\textsc{Methods} &  seen & unseen & drop \\ 
\hline
\hline
\textsc{VL Seq2Seq (SF)} & 38.6 & 21.8 & 16.8 \\
\hline
\textsc{RCM} &  67.4 &  42.5 & 24.9  \\
\hline
\textsc{Speaker-Follower} & 70.1 & 54.6 & 15.5 \\
\hline
\textsc{VLN Bert$^\dag$} & 71.8 & 54.5 & 17.3 \\
\hline
\hline
\textsc{Blind Agent} & 55.0 & 43.2 &  11.8 \\
\hline
\textsc{Blind Agent (M)} & 55.9 & 45.6 & \textbf{10.3} \\
\cline{1-4}
\end{tabular}
\caption{Comparison with Visual Methods on the R2R Dataset. We present the success rate (\texttt{SR}) of state-of-the-art visual methods and our method. $\dag$: Reimplemented without pretaining on the val\_unseen set. (M): Multi-Task model, see \cref{sec:multitask} for details.}
\label{tab:comp_vis}
\vspace{-3mm}
\end{table}


\vspace{-2mm}
\subsection{Towards Pure GPT-4-based Navigation?} 
In preliminary experiments, we found that just using prompted GPT-4 as the navigation agent (instead of finetuning LLaMA) did not work well. However, recent contemporaneous work \cite{zhou2023navgpt} finds that GPT-4 prompted with text descriptions can perform nontrivially when combined with chain-of-thought prompts \cite{nye2021scratch,wei2022cot}. While we were focused on training smaller open-source large language models, it would thus be interesting to see if both approaches can be combined (e.g., by distilling the chain-of-thought to smaller models that could be finetuned). 


==> tables/appx_ablation.tex <==


\begin{table*}[t]
\caption{
Ablation Study on the number of GPT-4 Generated Trajectories. The column headers provide the following information: \textsc{\# real} represents the number of realistic trajectories, \textsc{\# syn.} indicates the number of synthetic trajectories, and \textsc{src} denotes the source of the synthetic trajectories.}
\centering
\scalebox{0.9}{
\begin{tabular*}{\textwidth}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \toprule
\cline{1-13}
\multirow{2}{*}{\textsc{\# real}} & \multirow{2}{*}{\textsc{\# syn.}} & \multirow{2}{*}{\textsc{src}}  & \multicolumn{5}{c|}{\textit{R2R Seen}} & \multicolumn{5}{c|}{\textit{R2R Unseen}} \\ 
% \cmidrule(lr){3-7} \cmidrule(lr){8-12}  
\cline{4-13}
 &  & & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{OSR$\uparrow$} & \texttt{SPL$\uparrow$} & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{OSR$\uparrow$} & \texttt{SPL$\uparrow$}  \\ 
% \midrule
\cline{1-13}
\cline{1-13}

10 & 50 & GPT-4 & 9.6 & 9.6 & 11.4 & 19.7 & 9.7 & 9.5 & 9.4 & 13.3 & 20.6 & 11.3 \\
\cline{1-13}
10 & 100 & GPT-4 & 10.5 & 9.6 & 13.2 & 23.1 & 10.8 & 10.4 & 9.0 & 17.0 & 28.6 & 14.4 \\
\cline{1-13}
10 & 500 & GPT-4 & 9.1 & 8.2 & 21.3 & 26.8 & 18.9 & 9.0 & 7.9 & 22.6 & 29.9 & 20.7 \\

\cline{1-13}
\end{tabular*}
}
\label{tab:gpt4-abl}
\end{table*}



==> tables/appx_comparison.tex <==
\begin{table*}[t]
\centering
\captionof{table}{Comparison with Visual Methods on the R2R Dataset. $\dag$: Reimplemented without pretaining on the val\_unseen set. $\star$: Involved pre-training on the val\_unseen set, not directly comparable to our method. \textsc{($2\times$):} Ran each demonstration for twice when generating instruction-following pairs. \textsc{(M)}: Multi-Task model, see \cref{sec:multitask}. }
\begin{tabular*}{0.943\textwidth}{|c|c|c|c|c|c|c|c|c|c|c|}%{lllllll}
\cline{1-11}
\multirow{2}{*}{\textsc{Methods}} &  \multicolumn{4}{c|}{\textit{R2R Validation Seen}} & \multicolumn{4}{c|}{\textit{R2R Validation Unseen}} & \multicolumn{2}{c|}{\textit{SR Drop}} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11}
\cline{2-11}
 & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{SPL$\uparrow$} & \texttt{TL} & \texttt{NE$\downarrow$} & \texttt{SR$\uparrow$} & \texttt{SPL$\uparrow$} & \texttt{SR} & \texttt{SPL} \\ 
\hline
\hline
\textsc{Seq-to-Seq (SF)} & 11.3 & 6.0 & 38.6 & - &  8.4 & 7.8 & 21.8 & - & 16.8 & - \\
\cline{1-11}
\textsc{RCM} & 11.9 & 3.4 & 67.4 & - & 14.8 & 5.9 & 42.5 & - & 24.9 & - \\
\cline{1-11}
% \cmidrule(lr){1-1} \cmidrule(lr){2-9} 
\textsc{RCM + SIL (train)} & 10.7 & 3.5 & 66.7 & - & 11.5 & 6.1 & 42.8 & - & 23.9 & - \\
\cline{1-11}
\textsc{Speaker-Follower} & - & 3.1 & 70.1 & - & - & 4.8 & 54.6 & - & 15.5 & - \\
\cline{1-11}
\textsc{VLN Bert$^\dag$} & 10.9 & 3.2 & 71.8 & 68.2 & 12.1 & 5.0 & 54.5 & 49.0 & 17.3 & 19.2\\
\hline
\hline
\textsc{Blind Agent} & 11.1 & 5.5 & 49.1 & 45.8 & 12.6 & 6.3 & 40.1 & 35.9 & \textbf{9.0} & \textbf{9.9} \\
\cline{1-11}
\textsc{Blind Agent ($2\times$)} & 11.7 & 4.9 & 55.0 & 51.0 & 13.7 & 6.0 & 43.2 & 37.9 & 11.8 & 13.1 \\
\cline{1-11}
\textsc{Blind Agent (M)}  & 11.9 & 4.8 & 55.9 & 51.7 & 13.7 & 5.9 & 45.6 & 40.0 & 10.3 & 11.4 \\
\hline
\hline
\textsc{PREVALENT$^\star$}  & 10.3 & 3.7 &  69.0 & 65.0 & 10.2 & 4.7 & 58.0 & 53.0 & 11.0 & 12.0 \\
\cline{1-11}
\textsc{VLN Bert$^\star$}  & 11.1 & 2.9 & 72.0 & 68.0 & 12.0 & 3.9 & 63.0 & 57.0 & 11.0 & 11.0\\
\cline{1-11}
\end{tabular*}
\label{tab:r2r}
\end{table*}
